Cosmology at the Field Level with Probabilistic Machine Learning

The large-scale structure in cosmology is highly non-Gaussian at late times and small length scales, making it difficult to describe analytically. Parameter inference, data reconstruction, and data generation tasks in cosmology are greatly aided by various machine learning models. In order to retain as much information as possible while solving these problems, this work operates at the field level, rather than at the level of summary statistics. The probability density function of the large-scale structure is learned with normalizing flows, a class of probabilistic generative models. Normalizing flows learn the transformation from a simple base distribution to a more complicated distribution, much like the matter content evolved to its present day complexities from a Gaussian field at early times. While the normalizing flows have accurately modelled 2-dimensional projections of the matter content, we find that denoising diffusion models are well-suited for volumetric data. A super-resolution emulator is developed for cosmological simulation volumes, generating high-resolution baryonic simulation volumes conditional on low-resolution dark matter simulations. The super-resolution emulator is trained to perform outpainting, and can thus upgrade very large cosmological volumes from low-resolution to high-resolution using an iterative outpainting procedure.

==> chapters/forward.tex <==
\interfootnotelinepenalty=10000

New technology, machine learning. The research in this work is one small use case of this technology. We have gone through society changing technology several times in the past century. Integrated circuits and atomic physics. But unlike  computers in the 1960s, or enriched uranium in the 1940s, the general public has intimate access to machine learning technology as it is developed.

The use cases for nefarious purposes are vast. Trillion dollar companies sell our data to secret advertising agencies~\footnote{Authors. Title. \textit{Newspaper}, year.}.
Public facing businesses use facial recognition to identify and physically remove people they don't like~\footnote{Kasmir Hill. Madison Square Garden Uses Facial Recognition to Ban Its Owner’s Enemies. \textit{The New York Times}, 2022.}.
Police departments secretly use software they don't understand to attempt to predict crimes and set probation guidelines~\footnote{Cade Metz and Adam Satariano. An Algorithm That Grants Freedom, or Takes It Away. \textit{The New York Times}, 2020.}, and there is no judicial oversight on mass facial recognition surveillance~\footnote{Authors. Title. \textit{Journal}, year}.
Companies in the largest economic adversary to the United States harvest our data through malware disguised as social media~\footnote{Kristen E. Busch. TikTok: Recent Data Privacy and National Security Concerns. \textit{Congressional Research Service Reports}, IN12131, 2023.}.
A company named ``OpenAI" hides basic information about their flagship product~\footnote{OpenAI. GPT-4 Technical Report. \textit{arXiv e-prints}, arXiv:2303.08774, 2023.}.
The price of ordering a coffee on your phone is having your location secretly tracked 24/7~\footnote{Ian Austen. ‘A Mass Invasion of Privacy’ but No Penalties for Tim Hortons. \textit{The New York Times}, 2022.}.
Your vaccuum cleaner maps your home's floor plan, the rights to which were legally signed away when the vacuum turned on~\footnote{Maggie Astor. Your Roomba May Be Mapping Your Home, Collecting Data That Could Be Shared. \textit{New York Times}, 2017.}.
If a company or government agency has the opportunity to learn everything about every individual they come into contact with, they're going to.

The harm to the general public is more than simply companies are bad. There's an culture of distrust and conspiratorial thinking surrounding machine learning technology, and this hinders adoption of actual benefits of the technology. The public does not trust self-driving vehicles~\footnote{Lee Rainie, Cary Funk, Monica Anderson and Alec Tyson. AI and Human Enhancement: Americans’ Openness Is Tempered by a Range of Concerns. \textit{Pew Research Center}, 2022.}, even though they are almost always safer than human drivers~\footnote{Authors. Title. \textit{Journal}, year.}.

Our failure to properly understand and respond to recent advances in machine learning is one small part of an overarching cult of ignorance. More than a quarter of the United States lives in a desert with diminish water reserves, and more than a third live in an alternate reality where the laws of thermodynamics magically do not apply~\footnote{Cary Funk. Why Some Americans Do Not See Urgency on Climate Change. \textit{Pew Research Center}, 2023.}. We have State sponsored lotteries to capitalize on people's lack of basic arithmetic skills. More than one-fourth of the population has decided to throw a fundamental law of nature, the principle of locality, out the window in favor of astrology~\footnote{Becka A. Alper et al. The Religious Typology. \textit{Pew Research Center}, 2018.}. We distract ourselves with culture wars while corporations corner the housing market~\footnote{Francesca Mari. A \$60 Billion Housing Grab by Wall Street \textit{New York Times}, 2020.}.  We wonder why the birth rate has fallen faster than predicted in a country that provides no parental leave, no affordable daycare system, and no affordable higher education.

How does we tell ourselves to get out of these problems? Buy an AI day trader. Use a search engine optimization AI to boost your drop shipping pyramid scheme.

Companies mislead their investors by solving every problem with a vague ``AI solution." They are replacing customer service flowcharts that don't work with customer service large language models that don't work slightly less.

%I do not use the phrase ``artificial intelligence" in this work after the Forward. There is nothing intelligent about mapping data to other data. This research, and essentially all other research with machine learning, use mathematics to learn mappings between data sets with the help of modern computer hardware. The first step in understanding a new technology is to demystify it.

There seems to be no The United States spends half of one percent of its budget on NASA. We have a half-built and abandoned Superconducting Super Collider outside of Dallas. The Unites States clearly has a limited interest in being a world leader in the physical sciences.

The dichotomy of living in the wealthiest country on Earth, and not being able to do basic things. I can tell you the fundamental equations that govern the evolution of the Universe, but I can't . I can train a machine learning program to speak in English almost indistinguishably from a human, but I can't visit a dentist. 

The United States is failing its people, and machine learning will be used to aid in our decline.
We refuse to adaquately pay our teachers, and will replace them with large language models. We are automating our domestic shipping industry, and failing to provide for communities whose economy is propped up by a truck stop.
We will widen the wealth gap with investors' use of machine learning to corner the housing market.
We will dupe ourselves with false images and videos.
Our political biases are understood by social media companies better than ourselves, and are exploited by fine-tuned algorithms.
We will use computational geology to optimize oil pipeline development locations as we fail to migrate millions from the deserts of Arizona and the shores of Florida.
We will spend our resources mastering autonomous weapons technology so we may kill specific individuals on the other side of the world with almost no human intervention while our poor diabetes patients ration their insulin.
We will watch the rest of the developed world enter a new age of prosperity, as we choose to slip into the darkness.

==> chapters/sr_with_flow.tex <==
A conditional real NVP normalizing flow is used to generate super-resolution fields conditional on low-resolution fields. A patching procedure is used to do super-resolution on large low-resolution fields.


\section{Introduction}


Introduction

SRFlow \cite{SRFlow}, an extension of SRFlow \cite{SRFlowDA}

A grid scheme was used in \cite{Han_2021} by averaging overlapping regions in the small maps; however, we avoid taking such an average neighboring fields.


\section{Super-resolution with a conditional real NVP flow}


Sample and compute the PDF of super-resolution fields $\pmb{y}$ conditional on low-resolution fields $\pmb{x}$. 

\begin{equation}
    P{(\pmb{y}|\pmb{x})}=T_K\circ\cdots\circ T_1(\pmb{u},\pmb{\theta})
\end{equation}

The real NVP flow is made to be conditional on a low-resolution field. Fig.~\ref{fig:RNVP_sr_tikz}.

\begin{figure}[h]
\centering
\begin{tikzpicture}[node distance=0.65cm]
\footnotesize

\pgfdeclarelayer{bg}
\pgfsetlayers{bg, main}

\node[align=center, font=\bfseries] (title){Conditional real NVP};
\node (start) [cnn, below of=title] {Training data};
\node (params) [cnn, right of=start, xshift=9em, minimum width=1cm, align=center] {Low-resolution\\field};
\node (cb0) [cnn, below of=start, fill=black!15] {Checkerboard mask};
\node (cnn0) [cnn, below of=cb0, fill=azul!75] {$s,t$ CNN};
\node (at0) [cnn, below of=cnn0, fill=orange!30] {Affine transformation};
\node (end) [cnn, below of=at0, fill=red!0] {Gaussian field};

\draw [arrow] (start.east) to [out=-30,in=30](cb0.east);
\draw [arrow] (params.south) to [out=-90,in=0](cnn0.east) node[]{\hspace{4cm}Concatenate};
\draw [arrow] (cb0.east) to [out=-30,in=30](cnn0.east);
\draw [arrow] (cnn0.east) to [out=-30,in=30](at0.east);
\draw [arrow] (at0.west) to [out=135,in=-135](cb0.west) node[yshift=-0.68cm] {\hspace{-1.3cm}$\times K$};
\draw [arrow] (at0.east) to [out=-30,in=30](end.east);

\end{tikzpicture}
\hspace{0.5cm}
\begin{tikzpicture}[node distance=0.65cm]
\footnotesize

\pgfdeclarelayer{bg}
\pgfsetlayers{bg, main}

\node[align=center, font=\bfseries] (title){Reverse conditional real NVP};
\node (start) [cnn, below of=title] {Gaussian field};
\node (params) [cnn, right of=start, xshift=9em, minimum width=1cm, align=center] {Low-resolution\\field};
\node (cb0) [cnn, below of=start, fill=black!15] {Checkerboard mask};
\node (cnn0) [cnn, below of=cb0, fill=azul!75] {$s,t$ CNN};
\node (at0) [cnn, below of=cnn0, fill=orange!30] {Inv. affine transformation};
\node (end) [cnn, below of=at0, fill=red!0] {Generated data};

\draw [arrow] (start.east) to [out=-30,in=30](cb0.east);
\draw [arrow] (params.south) to [out=-90,in=0](cnn0.east) node[]{\hspace{4cm}Concatenate};
\draw [arrow] (cb0.east) to [out=-30,in=30](cnn0.east);
\draw [arrow] (cnn0.east) to [out=-30,in=30](at0.east);
\draw [arrow] (at0.west) to [out=135,in=-135](cb0.west) node[yshift=-0.68cm] {\hspace{-1.3cm}$\times K$};
\draw [arrow] (at0.east) to [out=-30,in=30](end.east);

\end{tikzpicture}

\ 

\begin{tikzpicture}[node distance=0.65cm]
\footnotesize

\node[align=center, font=\bfseries] (title){$\pmb{s},\pmb{t}$ CNN};
\node (conv0) [cnn, below of=title] {Image: $2\times n^2$};
\node (conv1) [cnn, below of=conv0, fill=azul!75] {$3\times3$ conv: $c\times n^2$};
\node (conv2) [cnn, below of=conv1, fill=azul!75] {$3\times3$ conv: $c\times n^2$};
\node (conv3) [cnn, below of=conv2, fill=azul!75] {$3\times3$ conv: $2\times n^2$};
\node (st) [cnn, below of=conv3] {$s,t$: $2\times n^2$};

\draw [arrow] (conv0.east) to [out=-30,in=30](conv1.east);
\draw [arrow] (conv1.east) to [out=-30,in=30](conv2.east) node[yshift=0.35cm] {\hspace{2.4cm}Leaky ReLU};
\draw [arrow] (conv2.east) to [out=-30,in=30](conv3.east) node[yshift=0.35cm] {\hspace{2.4cm}Leaky ReLU};
\draw [arrow] (conv3.east) to [out=-30,in=30](st.east) node[yshift=0.35cm] {\hspace{1.3cm}Tanh};

\end{tikzpicture}

\caption[A real NVP normalizing flow conditional on a low-resolution field]{(Top left) A real NVP flow conditional on a low-resolution field. (Bottom) The CNN has a $2$ channel input to include a low-resolution field concatenated along channels with the training data, or with the Gaussian field in the reverse direction.}
\label{fig:RNVP_sr_tikz}
\end{figure}


%\section{Mode coupling}


%The PDF is learned with a normalizing flow, allowing gradients
%\begin{equation}
%    \nabla_{\pmb{x}_\text{long}}p{(\pmb{x}_\text{short}|\pmb{x}_\text{long})}
%\end{equation}
%of it to be taken, and thus the PDF can be extremized for a MAP solution $\pmb{x}_\text{long}$.


\section{Iterative patching to operate on large fields}


An iterative patching scheme is explained to do super-resolution on large low-resolution fields. Fig.~\ref{fig:patching_2d}

\begin{figure}
    \centering
    \includegraphics[width=0.37\textwidth]{images/grid_scheme_2d.png}
    \hspace{0.75cm}
    \includegraphics[width=0.37\textwidth]{images/conditional_example_2d.png}
    \caption[Super-resolution on large fields accomplished by iteratively doing super-resolution on small patches]{Super-resolution on large fields is accomplished by iteratively doing super-resolution on small patches. (Left) An illustration of the patching scheme in 2 spacial dimensions. (Right) The low-resolution fields are small patches with a super-resolution conditional border.}
    \label{fig:patching_2d}
\end{figure}


\section{Results on large n-body simulations with patching}


Here we show results on 2-dimensional projections of n-body simulations. We 


\section{Conclusion}


Mode coupling, learning long length modes from observed short length modes. $p{(\pmb{x}_\text{short}|\pmb{x}_\text{long})}$. The PDF can be extremized for a MAP solution $\pmb{x}_\text{long}$.

The results in 3 spacial dimensions were inaccurate, with the flow not being able to learn the small length scale modes. In the next chapter, a conditional denoising diffusion model is used for 3-dimensional data.
